Fast Inference for Augmented Large Language Models

Augmented Large Language Models (LLMs) enhance the capabilities of standalone LLMs by integrating external data sources through API calls. In interactive LLM applications, efficient scheduling is crucial for maintaining low request completion times, directly impacting user engagement. However, these augmentations introduce scheduling challenges due to the need to manage limited memory for cached information (KV caches). As a result, traditional size-based scheduling algorithms, such as Shortest Job First (SJF), become less effective at minimizing completion times. Existing work focuses only on handling requests during API calls by preserving, discarding, or swapping memory without considering how to schedule requests with API calls. In this paper, we propose LAMPS, a novel LLM inference framework for augmented LLMs. LAMPS minimizes request completion time through a unified scheduling approach that considers the total length of requests and their handling strategies during API calls. Recognizing that LLM inference is memory-bound, our approach ranks requests based on their consumption of memory over time, which depends on both the output sizes and how a request is managed during its API calls. To implement our scheduling, LAMPS predicts the strategy that minimizes memory waste of a request during its API calls, aligning with but improving upon existing approaches. We also propose starvation prevention techniques and optimizations to mitigate the overhead of our scheduling. We implement LAMPS on top of vLLM and evaluate its performance against baseline LLM inference systems, demonstrating improvements in end-to-end latency by 27%-85% and reductions in TTFT by 4%-96% compared to the existing augmented-LLM system, with even greater gains over vLLM.

==> removed.tex <==
- Due to the large GPU memory footprint and compute cost of LLMs, serving dominates the compute cost for most real world applications. ML engineers often treat LLMs like "black boxes" that can only be optimized with internal changes such as quantization and custom CUDA kernels. However, this is not entirely the case. Because LLMs iteratively generate their output, and because LLM inference is often memory and not compute bound, there are



\begin{comment}
    Introduction to the Scheduling Challenge in LLMs

Briefly introduce the importance of efficient scheduling in large language models (LLMs).
Highlight the complexities and unique challenges posed by varying request types and workloads.
The Need for Effective Request Handling in Scheduling

Explain that proper scheduling relies on understanding how to handle each individual request efficiently.
Emphasize that without tailored handling, scheduling cannot optimize performance or resource utilization.
Minimizing Memory Waste as a Key to Efficient Handling

Discuss how memory constraints, particularly regarding the key-value (KV) cache, impact LLM performance.
Argue that minimizing memory waste is crucial for handling requests effectively.
Predicting Request Properties to Optimize Handling

Introduce the idea of predicting properties such as output length, computational load, or memory requirements.
Explain how accurate predictions enable more efficient handling of each request.
From Prediction to Optimized Scheduling

Show how knowing the predicted properties informs scheduling decisions.
Describe how this leads to better resource allocation, reduced latency, and improved overall system performance.
Opportunity for Advanced Scheduling Policies

Highlight the potential to develop new scheduling policies that incorporate request predictions.
Mention that this approach can address current limitations, such as those in systems without API augmentations.
Conclusion

Summarize how understanding and predicting request properties transforms the scheduling challenge into an opportunity.
Suggest directions for future research or implementation based on this approach.
\end{comment}


\textbf{Challenge.} Handling API-augmented requests poses a challenge due to the need to maintain key-value caches in GPU memory, which has limited capacity. During API calls, this valuable memory could be wasted instead of accommodating other requests, potentially increasing latency and reducing throughput.

\textbf{Memory management during API calls.} Three strategies address this challenge:
\begin{enumerate}
    \item ``Discard'', the traditional approach used by existing LLM inference systems~\cite{}, treats an API call as a termination signal. It concludes the ongoing request, discards its context, delegates the task to the augmenting entity, and initiates a new request upon receiving the response. This method leads to substantial recomputation of the KV cache from the start, wasting GPU resources that could serve new requests.
    \item The ``Preserve'' strategy maintains the context of a request during the API call and resumes the request when the call finishes. While this avoids recomputation, it occupies GPU memory throughout the entire API call.
    \item The ``Swap'' strategy moves contexts to CPU memory during API calls. This method avoids both recomputation and GPU memory waste. However, the limited bandwidth of the GPU-CPU link could bottleneck foreground tasks as they wait for swapping to complete.
\end{enumerate}

The optimal strategy for memory management during API calls should aim to minimize wasted memory, as this is the most critical metric in inference. For relatively brief API durations, preserving the request may be preferable. However, for extended API calls, we have two options: discard and recompute, or swap. {\bf MM: make these overheads clearer above and avoid repeating;  what does "impact the forward pass" mean other than what was said above?}
Each option carries its own overhead. Discarding requires re-computation of the pre-API call part while swapping impacts the model's forward pass. As a rule of thumb, if the pre-API portion is ``short'' (computationally light), discarding is preferable; otherwise, swapping may be the better choice.

{\bf MM: "their equations" comes a bit out of the blue;  make clearer they develop equations that model "memory wastage" of each strategy?}
This explanation offers a high-level intuition as other components of the system also influence memory usage.
Infercept~\cite{} quantifies the memory waste associated with each strategy, and their equations reflect this intuition while accounting for additional factors. Infercept dynamically selects the approach that minimizes waste for individual requests. When a request encounters an API call, Infercept calculates its potential memory waste in real-time and applies the most efficient strategy accordingly.
However, this runtime decision-making approach, while effective for the currently scheduled requests, misses opportunities for optimizing the overall system. If we knew the optimal strategy for each request in advance, we could schedule and prioritize them differently to minimize average end-to-end latency.
{\bf MM: would be good to give some intuition/example, not clear why knowing in advance is better than dynamic response from this.}





\subsection{Scheduling API-augmented requests}
To ensure an engaging experience for users, the interactive nature of LLM applications demands a low job completion time (JCT) for inference. However, traditional scheduling methods face challenges with API-augmented requests. First Come First Served (FCFS), currently employed by traditional inference systems~\cite{}, and Shortest requests First (SJF) (even assuming known output lengths)\footnote{In the examples, we assume an offline setting for simplicity.} fail to perform optimally when requests involve API calls.


Example. Figure~\ref{fig:example} illustrates the baseline schedulers and highlights the challenges when API calls are included in the requests. 

Three requests arrive at time $0$ in the order of $J_1$, $J_2$, $J_3$, where all have one API call triggered at different times during decode generation. Their output lengths are 9, 2, and 3, respectively, and the API durations (in token generation units) are 2, 10, and 2, respectively. Table~\ref{tab:example_durations} summarizes the total length of the request (prefill + decode) and the API duration for these requests.

{\bf MM: Is this example assuming only one job can run at a time?  Make explicit.  Maybe also make clearer that FCFS/SJF in this example do not take into account memory action;  rather, scheduling "comes first", and memory-based policy is determined by Infercept equations?}

{\bf MM: High-level comment:  make clearer the ordering of decision:  you can either have a scheduling policy [like FCFS] and decide memory dynamically;  or you can decide memory policy first, and schedule with that info.  (I suppose a third option is "co-schedule" with scheduling policy+memory together, but that's complicated/may require offline to do well.)}

Based on our intuition about memory management during API calls, we assume the following strategies: preserve for $J_1$, discard for $J_2$, and swap for $J_3$. Considering a batch size of 1, the average JCT for First-Come-First-Serve (FCFS), which is used by Infercept, is 17, while Shortest Job First (SJF) yields 12.3 (Figures~\ref{fig:example_fcfs} and~\ref{fig:example_job}, respectively).

These baseline approaches, however, do not achieve optimal scheduling, even when appropriately managing memory during API calls. A naive approach might order requests by their total length (output + API duration), which we refer to as "SJF by total length" (Figure~\ref{fig:example_job_api}). In this approach, we break ties by the index of the requests, yielding average JCT of 40. However, this example reveals a critical insight: 
{\bf MM:  Not equal, even under this metric?}
$J_1$ and $J_2$ have equal total lengths but should be treated differently due to their individual memory management strategies.


\textbf{RANA: update the example of FCFS and the other to consider w/w.o preemption}

Figure~\ref{fig:example_opt} demonstrates a scheduling approach that yields the optimal average JCT of 11.6, outperforming the previous methods. This optimal scheduling 'treats' requests based on both their total length and their memory management strategy. Specifically, when two requests have the same total length, but different management strategies, they are handled differently.






\subsection{Opportunities}

Previous examples demonstrate that prior knowledge of request lengths can lead to an improved average JCT.
The challenge comes in obtaining three key pieces of information: output length without API, API duration, and API output length.

Predicting the output length of prompts has been explored in previous research. $S^3$~\cite{jin2023s} fine-tunes a DistilBERT model~\cite{sanh2019distilbert}, originally trained for sequence classification, to categorize output sequence lengths into specific buckets. While Zheng et al.~\cite{zheng2024response} utilize the inherent response length perception abilities of LLMs. Both approaches focus on predicting the output sequence length but through different methods. Regarding API duration, the Infercept system takes a different approach by summarizing API properties based on their types, including mean duration and variance. This provides a comprehensive view of the expected API performance.

\todo[inline]{look on the following approaches..}

A significant challenge remains in predicting the length of API output. Unlike prompt-based language models, API output can vary significantly depending on the specific function and input parameters.
To address this challenge, we propose several potential approaches:

\begin{itemize}
    \item Historical data analysis: By collecting and analyzing historical data on API calls and their corresponding output lengths, we can develop statistical (ML) models to predict future output lengths.
    \item API metadata augmentation: API includes metadata about expected output sizes or ranges.
    \item Sampling: periodically sample API outputs and updates predictions in real-time. 
\end{itemize}



\begin{comment}
Augmented Large Language Models (LLMs) enhance standalone LLM capabilities by integrating external data sources through API calls. Efficient scheduling is crucial for maintaining low request completion times in interactive applications, especially in Augmented LLMs, where user engagement depends on responsiveness. However, these interactions introduce scheduling challenges due to increased memory overhead, which plays a critical role in LLM inference. As a result, traditional size-based scheduling algorithms, such as Shortest Job First (SJF), become less effective at minimizing completion times.
Existing work focuses only on handling requests during API calls by preserving, discarding, or swapping memory, without considering how to schedule requests with API calls.
In this paper, we propose \alg{}, a novel LLM inference framework for augmented LLMs. 
\alg{} minimizes request completion time through a unified scheduling approach that jointly considers the total length of requests and their API call handling strategies. Our approach ranks requests with varying output sizes and handling strategies during API calls according to their memory over time consumption.
To incorporate this into the scheduler before a request begins processing, \alg{} predicts the pre-API output length and duration of the API call and optimizes the handling of requests during API calls to minimize memory waste, aligning with existing approaches.
We prove the optimality of a scheduling policy that ranks requests based on the area under their memory-over-time curves, representing total memory consumption over a request's processing time. We implement \alg{} on top of vLLM and compare its performance against baseline scheduling algorithms, \rana{TODO: add evaluation numbers}
\end{comment}


\begin{figure*}[ht!]
    \centering
    \begin{tikzpicture}
        % Column labels
        \node at (5.5, 12) {\textbf{Model 6B}};
        \node at (14.5, 12) {\textbf{Model 13B}};
        
        % Row labels
        \node[rotate=90] at (1, 9) {\textbf{Single}};
        \node[rotate=90] at (1, 4) {\textbf{Multi}};
        \node[rotate=90] at (1, -1) {\textbf{ToolBench}};

        % Separator between the two columns
        \draw[dashed, gray, very thin] (10, 11) -- (10, -2);

        % Legend (adjust position as needed)
        \node at (10, -4) {
            \begin{minipage}{0.6\textwidth}
                \centering
                \includegraphics[width=\textwidth]{eval_graphs/performance/strategy_legend.pdf}
            \end{minipage}
        };
        % First row of subfigures (Single API)
        \node at (5.5, 9) {
            \begin{minipage}{0.5\linewidth}
                \centering
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/6B/Single API_6B_1800_E2E Latency_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/6B/Single API_6B_1800_E2E Latency_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/6B/Single API_6B_1800_E2E Latency_P99.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/6B/Single API_6B_1800_TTFT_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/6B/Single API_6B_1800_TTFT_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/6B/Single API_6B_1800_TTFT_P99.pdf}
            \end{minipage}
        };
        \node at (14.5, 9) {
            \begin{minipage}{0.5\linewidth}
                \centering
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/13B/Single API_13B_1800_E2E Latency_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/13B/Single API_13B_1800_E2E Latency_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/13B/Single API_13B_1800_E2E Latency_P99.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/13B/Single API_13B_1800_TTFT_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/13B/Single API_13B_1800_TTFT_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/13B/Single API_13B_1800_TTFT_P99.pdf}
            \end{minipage}
        };

        % Second row of subfigures (Multi API)
        \node at (5.5, 4) {
            \begin{minipage}{0.5\linewidth}
                \centering
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/mult_api/6B/Multi API_6B_1800_E2E Latency_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/mult_api/6B/Multi API_6B_1800_E2E Latency_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/mult_api/6B/Multi API_6B_1800_E2E Latency_P99.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/mult_api/6B/Multi API_6B_1800_TTFT_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/mult_api/6B/Multi API_6B_1800_TTFT_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/mult_api/6B/Multi API_6B_1800_TTFT_P99.pdf}
            \end{minipage}
        };
        \node at (14.5, 4) {
            \begin{minipage}{0.5\linewidth}
                \centering
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/mult_api/13B/Multi API_13B_1800_E2E Latency_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/mult_api/13B/Multi API_13B_1800_E2E Latency_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/mult_api/13B/Multi API_13B_1800_E2E Latency_P99.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/mult_api/13B/Multi API_13B_1800_TTFT_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/13B/Single API_13B_1800_TTFT_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/single_api/13B/Single API_13B_1800_TTFT_P99.pdf}
            \end{minipage}
        };

        % Third row of subfigures (ToolBench Latency)
        \node at (5.5, -1) {
            \begin{minipage}{0.5\linewidth}
                \centering
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/6B/Multi API_6B_1800_E2E Latency_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/6B/Multi API_6B_1800_E2E Latency_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/6B/Multi API_6B_1800_E2E Latency_P99.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/6B/Multi API_6B_1800_TTFT_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/6B/Multi API_6B_1800_TTFT_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/6B/Multi API_6B_1800_TTFT_P99.pdf}
            \end{minipage}
        };
        \node at (14.5, -1) {
            \begin{minipage}{0.5\linewidth}
                \centering
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/13B/Multi API_13B_1800_E2E Latency_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/13B/Multi API_13B_1800_E2E Latency_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/13B/Multi API_13B_1800_E2E Latency_P99.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/13B/Multi API_13B_1800_TTFT_Mean.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/13B/Multi API_13B_1800_TTFT_Median.pdf}
                \includegraphics[width=0.3\linewidth]{eval_graphs/performance/toolbench/13B/Multi API_13B_1800_TTFT_P99.pdf}
            \end{minipage}
        };
    \end{tikzpicture}
    \caption{Comparison of results for different models and datasets.}
\end{figure*}



\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.325\linewidth}
        \centering
        \includegraphics[width=\textwidth]{eval_graphs/performance/mult_api/6B/starvation_prevension/Multi API_6B_1800_Throughput.pdf}  % Replace with your figure
        \caption{Single-API}
        \label{fig:starvation1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \centering
        \includegraphics[width=\textwidth]{eval_graphs/performance/mult_api/13B/Multi API_13B_1800_Throughput.pdf}  % Replace with your figure
        \caption{Multi-API}
        \label{fig:starvation2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.325\linewidth}
        \centering
        \includegraphics[width=\textwidth]{eval_graphs/performance/toolbench/13B/Multi API_13B_1800_Throughput.pdf}  % Replace with your figure
        \caption{ToolBench}
        \label{fig:starvation3}
    \end{subfigure}
    \includegraphics[width=0.7\linewidth]{eval_graphs/performance/strategy_legend.pdf}
    \caption{}
    \label{fig:starvation}
\end{figure}



\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\textwidth]{eval_graphs/performance/mult_api/6B/starvation_prevension/Multi API_6B_1800_Throughput.pdf}
        \label{fig:err_starvation_throughput}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\linewidth}
        \centering
        \includegraphics[width=\textwidth]{eval_graphs/performance/mult_api/6B/starvation_prevension/Multi API_6B_1800_P99_E2E Latency.pdf}
        \label{fig:err_starvation_latency}
    \end{subfigure}
    \includegraphics[width=\linewidth]{eval_graphs/performance/mult_api/6B/starvation_prevension/strategy_legend.pdf}
    \caption{}
    \label{fig:starvation}
\end{figure}

==> sections/explainations.tex <==
\section*{Computation Time Analysis in Transformer Models}

In transformer models, the computation time can be divided into two main components: prefill and decode. The complexities of these components are influenced by the sequence length and the model dimensionality.

\subsection*{Prefill Computation Time}

The prefill phase involves computing the self-attention for the given prompt. The time complexity for self-attention in transformers is typically \( O(n^2 \cdot d) \), where \( n \) is the sequence length and \( d \) is the model dimensionality.

For a prompt of length \( n_{\text{prefill}} \):

\[
T_{\text{prefill}} = k_1 \cdot n_{\text{prefill}}^2 \cdot d
\]

where \( k_1 \) is a constant factor representing the time per unit of computation for the self-attention mechanism.

\subsection*{Decode Computation Time}

The decode phase involves generating each token in an autoregressive manner. For each token generation, the model performs self-attention over the entire sequence generated so far, which includes the prompt and all previously generated tokens.

The time complexity for generating the \( i \)-th token is:

\[
O((n_{\text{prefill}} + i)^2 \cdot d)
\]

where \( i \) is the position of the token in the output sequence.

Summing this over all \( n_{\text{decode}} \) tokens gives:

\[
T_{\text{decode}} = \sum_{i=1}^{n_{\text{decode}}} k_2 \cdot (n_{\text{prefill}} + i)^2 \cdot d
\]

where \( k_2 \) is a constant factor representing the time per unit of computation for the decode process.

\subsection*{Total Computation Time}

The total computation time \( T_{\text{total}} \) is the sum of the prefill and decode computation times:

\[
T_{\text{total}} = T_{\text{prefill}} + T_{\text{decode}}
\]

Substituting the expressions for \( T_{\text{prefill}} \) and \( T_{\text{decode}} \):

\[
T_{\text{total}} = k_1 \cdot n_{\text{prefill}}^2 \cdot d + \sum_{i=1}^{n_{\text{decode}}} k_2 \cdot (n_{\text{prefill}} + i)^2 \cdot d
\]

This expression captures the computational cost of processing the initial prompt (prefill) and generating the subsequent tokens (decode), highlighting the dependencies on both the length of the prompt and the length of the generated sequence.


==> sections/theory.tex <==

%{\bf MM: I think this theorem statement needs to be clearer;  this is for a finite number of jobs?  $D_i$ is not really a "value" that depends on $i$;  it depends on the ordering chosen (similarly for the waiting time $W_i$, which is time until service begins, right?  So I think you need to have $W_i$, $D_i$ depend on the schedule ordering call it $S$, and consider an $S'$ from swapping. Use notation like $W_i(\mathcal{S}), W_i(S')$}

\begin{comment}
    
\begin{theorem}
\label{thm:ascending_memory_general}

In a system with unlimited servers, a finite number of requests and a finite total memory capacity $M_{total}$, where each request $i$ has a known service time $S_i$, memory consumption $M_i$, and may experience an additional delay $D_i$ due to memory constraints, scheduling requests in ascending order of $M_i$ minimizes the total response time. This approach is most effective when higher memory consumption generally aligns with longer service times, with rare exceptions.
\end{theorem}

\rana{edit theorem}
%, under the assumption that $M_i > M_j$ implies $S_i \geq S_j$.

Due to space constraints, the proof of Theorem~\ref{thm:ascending_memory_general} is provided in the appendix.
\end{comment}


\begin{comment}
\begin{proof}
    
We show that swapping any pair of adjacent requests on the same server, where a higher-memory request precedes a lower-memory one, along with corresponding adjustments on other servers, if necessary, does not increase the total response time.

We define the total response time for request $i$ under schedule $\mathcal{S}$ as $R_i(\mathcal{S}) = W_i(\mathcal{S}) + S_i + D_i(\mathcal{S})$ where $W_i(\mathcal{S})$ is the waiting time, $S_i$ is the service time, and $D_i(\mathcal{S})$ is the additional delay for request $i$ due to memory constraints. Let $M_i$ be the memory consumption of request $i$


The total response time is:
\[
T_{\text{total}} (\mathcal{S}) = \sum_{i} R_i(\mathcal{S}) = \sum_{i} (W_i(\mathcal{S}) + S_i + D_i(\mathcal{S}))
\]

Consider $\mathcal{S}$ schedule that is not in ascending order of $M_i$. At least one pair of adjacent requests exists where a higher-memory request $i$ precedes a lower-memory request $j$, i.e., $M_i > M_j$. Let $\mathcal{S^\prime}$ be schedule obtained by swapping $i$ and $j$.

Our goal is to show that $\mathcal{S^\prime}$ reduces (or does not increase) total response time.



Let $\Delta T_{\text{total}}$ be the change in total response time due to swapping $i$ and $j$ (between $\mathcal{S}$ and $\mathcal{S^\prime}$):
%{\bf MM: Why are only $i$ and $j$ affected?}

\[
\Delta T_{\text{total}} = T_{\text{total}} (\mathcal{S^\prime}) - T_{\text{total}} (\mathcal{S}) = \sum_{i} \Delta R_i
%(R_i^{\text{after}} + R_j^{\text{after}}) - (R_i^{\text{before}} + R_j^{\text{before}})
\]

%Where $$R_x^{\text{before/after}} = W_x^{\text{before/after}} + S_x + D_x^{\text{before/after}} \quad \text{for} \, x \in \{i, j\}$$

Where \( \Delta R_i = R_i(\mathcal{S^\prime}) - R_i(\mathcal{S})\).

\textbf{Changes for $i$ and $j$.}
For $i$ and $j$, the swap only affects their waiting times and additional delays while service times remain the same. In particular, the waiting time for the request $i$ increases by $S_j$.
\[
W_i({\mathcal{S^\prime}}) = W_i({\mathcal{S}}) + S_j
\]

The waiting time for the request $j$ decreases by $S_i$.
\[
W_j({\mathcal{S^\prime}}) = W_j({\mathcal{S}}) - S_i
\]

\textbf{Total change for $i$ and $j$:}

\begin{align*}
 = &\left[ (W_i({\mathcal{S}}) + S_j) + S_i + D_i({\mathcal{S^\prime}}) \right. \\
&\left. + (W_j({\mathcal{S}}) - S_i) + S_j + D_j({\mathcal{S^\prime}}) \right] \\
&- \left[ W_i({\mathcal{S}}) + S_i + D_i({\mathcal{S}}) + W_j({\mathcal{S}}) + S_j + D_j({\mathcal{S}}) \right] \\
& = \left[ S_j - S_i + D_i({\mathcal{S^\prime}}) + D_j({\mathcal{S^\prime}}) - D_i({\mathcal{S}}) - D_j({\mathcal{S}}) \right] \\
&= \Delta S + \Delta D_i + \Delta D_j
\end{align*}




\textbf{$\Delta D_i + \Delta D_j$:} 

After swapping, with $j$ processed before $i$, the cumulative memory consumption, which is the total memory used by all running requests (as requests complete, they free up memory), is lower when processing $j$. Thus, the additional delays $D_j({\mathcal{S^\prime}})$ and $D_i({\mathcal{S^\prime}})$ may be reduced or removed.


\[
D_i({\mathcal{S^\prime}}) \leq D_i({\mathcal{S}})
\]
\[
D_j({\mathcal{S^\prime}}) \leq D_j({\mathcal{S}})
\]
Thus: 
\[
\Delta D = (D_i({\mathcal{S^\prime}}) + D_j({\mathcal{S^\prime}})) - (D_i({\mathcal{S}}) + D_j({\mathcal{S}})) \leq 0
\]

%{\bf MM: I think you're stuck with this assumption;  you can put it in the theorem, and explain this shows that sorting in this way is "intuitively good"; 
%may not be perfect when this assumption is broken, but claim the assumption is rarely broken.  Maybe then provide experimental results if possible.}


\textbf{Changes for other Requests \( k \ne i, j \)}
Swapping \( i \) and \( j \) changes the cumulative memory usage profile of the system over time. By scheduling the lower-memory request \( j \) before the higher-memory request \( i \), the cumulative memory consumption at earlier times is reduced. This can lead to reduced delays for other requests that start during or after the time interval when \( j \) and \( i \) are processed may experience reduced delays \( D_k \) due to lower cumulative memory usage. Note that Since the positions of other requests relative to each other remain unchanged, their waiting times \( W_k \) remain the same.


Therefore, for each \( k \ne i, j \):

\begin{align*}
\Delta R_k &= R_k(S') - R_k(S) \\
           &= [W_k(S') - W_k(S)] + [D_k(S') - D_k(S)] + (S_k - S_k) \\
           &= \Delta D_k.
\end{align*}


since \( W_k(S') = W_k(S) \) and \( S_k \) remains the same.

Our goal is to show that \( \Delta D_k \leq 0 \) for all \( k \ne i, j \).


When we swap \( i \) and \( j \), the cumulative memory consumption at any time \( t \) becomes lower during the time when \( j \) is processed first, leading to a reduced cumulative memory usage at earlier times.

\[
D_k(S') \leq D_k(S) \implies \Delta D_k = D_k(S') - D_k(S) \leq 0.
\]

Thus, the delays for other requests \( k \ne i, j \) do not increase and may decrease due to the swap.



\paragraph{Total Change in Response Time}

The total change in response time is:

\[
\Delta T_{\text{total}} = \Delta R_i + \Delta R_j + \sum_{k \ne i,j} \Delta R_k = (S_j - S_i) + (\Delta D_i + \Delta D_j) + \sum_{k \ne i,j} \Delta D_k.
\]

Since \( \Delta D_k \leq 0 \) for all \( k \ne i, j \), and \( \Delta D_i + \Delta D_j \leq 0 \), we have:

\[
\Delta T_{\text{total}} \leq (S_j - S_i).
\]

\paragraph{A note on the assumption.}
While we generally assume that \( M_i > M_j \) implies \( S_i \geq S_j \), it is important to note that memory consumption \( M_i \) depends on both the service time \( S_i \) and the handling strategy applied during the API call (preserve, swap, or discard). Typically, requests with longer API duration are handled using swap or discard strategies to free up GPU memory. In contrast, requests with shorter service times may use the preserve strategy, keeping data in GPU memory and resulting in higher \( M_i \) but potentially lower \( S_i \). Therefore, there are rare cases where \( M_i > M_j \) but \( S_i < S_j \), such as when request \( i \) is handled by preserve and request \( j \) by swap. However, these exceptions are infrequent, and the assumption \( M_i > M_j \implies S_i \geq S_j \) generally holds in our system. Moreover, even when $\Delta S = S_j - S_i > 0$, the reduction in cumulative delay ($\Delta D$) often offsets this difference. Therefore, although the scheduling may not be perfect when the assumption is broken, it generally leads to minimized total response time in our system as shown in Section~\ref{sec:evaluation}.



Therefore:

\[
\Delta T_{\text{total}} \leq 0.
\]

\end{proof}
\end{comment}


